Performance Analysis of a Mass-Spring-Damper Deformable Linear Object Model in Robotic Simulation Frameworks

The modelling of Deformable Linear Objects (DLOs) such as cables, wires, and strings presents significant challenges due to their flexible and deformable nature. In robotics, accurately simulating the dynamic behavior of DLOs is essential for automating tasks like wire handling and assembly. The presented study is a preliminary analysis aimed at force data collection through domain randomization (DR) for training a robot in simulation, using a Mass-Spring-Damper (MSD) system as the reference model. The study aims to assess the impact of model parameter variations on DLO dynamics, using Isaac Sim and Gazebo to validate the applicability of DR technique in these scenarios.

==> styles/literature.tex <==
In this a geometrically consistent model of DLOs is developed and adopted to perform numerical simulations on the object motion under gravity and during the interaction with the environment.

A. Theetten, L. Grisoni, C. Andriot and B. Barsky, "Geometrically exact dynamic splines", Computer-Aided Design, vol. 40, no. 1, pp. 35-48, 2008.


In this a linearized spline-based DLO model called quasi dynamic splines is developed for the purpose of interaction simulation. 

 Theetten, L. Grisoni, C. Duriez and X. Merlhiot, "Quasi-dynamic splines", Proc. ACM Symposium on Solid and Physical Modeling, pp. 409-414, 2007.

 The integration of robotic vision and tactile sensing for switchgear cabling tasks is reported in
 D. De Gregorio, R. Zanella, G. Palli, S. Pirozzi and C. Melchiorri, "Integration of robotic vision and tactile sensing for wire-terminal insertion tasks", IEEE Tran. on Automation Science and Engineering, vol. 16, no. 2, pp. 585-598, 2018.

 Robotic manipulation and sensing of deformable objects in domestic and industrial applications: a survey:
Jose Sanchez,
Juan Antonio Corrales Ramon,
Belhassen-Chedli Bouzgarrou,
Youcef Mezouar
13 Jun 
2018
 - The International Journal of Robotics Re... 
Show Less
TL;DR: A survey of recent work on robot manipulation and sensing of deformable objects, a field with relevant applications in diverse industries such as medicine, food handling, manufacturing, and domestic chores, which is classified into four categories based on the type of object they manipulate.

Deformable Linear Objects 3D Shape Estimation and Tracking From Multiple 2D Views
Alessio Caporali,
Kevin Galassi,
Gianluca Palli
01 Jun 
2023
 - IEEE robotics and automation letters 
 - Vol. 8, pp 3851-3858
Show Less
PDF
Save
Cite

TL;DR: In this article , the authors presented DLO3DS, an approach for the 3D shapes estimation and tracking of Deformable Linear Objects (DLOs) using a cheap and compact 2D vision sensor mounted on the robot end-effector

Dynamic Manipulation of a Deformable Linear Object: Simulation and Learning
Qi Jing Chen,
+3 more
 - 
02 Oct 
2023
 - arXiv.org 
 - Vol. abs/2310.00911
PDF
Save
Cite

TL;DR: Dynamic manipulation of a deformable linear object (DLO) can be learned in simulation and transferred to real-world tasks without additional training.
Abstract: We show that it is possible to learn an open-loop policy in simulation for the dynamic manipulation of a deformable linear object (DLO) -- e.g., a rope, wire, or cable -- that can be executed by a real robot without additional training. Our method is enabled by integrating an existing state-of-the-art DLO model (Discrete Elastic Rods) with MuJoCo, a robot simulator. We describe how this integration was done, check that validation results produced in simulation match what we expect from analysis of the physics, and apply policy optimization to train an open-loop policy from data collected only in simulation that uses a robot arm to fling a wire precisely between two obstacles. This policy achieves a success rate of 76.7 percent when executed by a real robot in hardware experiments without additional training on the real task.
